Momentum exchange method for quantum Boltzmann methods

The past years have seen a surge in quantum algorithms for computational fluid dynamics (CFD). These algorithms have in common that whilst promising a speed-up in the performance of the algorithm, no specific method of measurement has been suggested. This means that while the algorithms presented in the literature may be promising methods for creating the quantum state that represents the final flow field, an efficient measurement strategy is not available. This paper marks the first quantum method proposed to efficiently calculate quantities of interest (QoIs) from a state vector representing the flow field. In particular, we propose a method to calculate the force acting on an object immersed in the fluid using a quantum version of the momentum exchange method (MEM) that is commonly used in lattice Boltzmann methods to determine the drag and lift coefficients. In order to achieve this we furthermore give a scheme that implements bounce back boundary conditions on a quantum computer, as those are the boundary conditions the momentum exchange method is designed for.

==> 2bounceback-wall-reflection.tex <==
\scalebox{1.0}{
\Qcircuit @C=1.0em @R=0.2em @!R { \\
	 	\nghost{{a\_v}_{0} :  } & \lstick{{a\_v}_{0} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw \barrier[0em]{15} & \qw & \ctrl{2} & \qw & \qw\\
	 	\nghost{{a\_v}_{1} :  } & \lstick{{a\_v}_{1} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{a\_o}_{0} :  } & \lstick{{a\_o}_{0} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \targ & \qw & \qw\\
	 	\nghost{{a\_o}_{1} :  } & \lstick{{a\_o}_{1} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{a\_c}_{0} :  } & \lstick{{a\_c}_{0} :  } & \multigate{7}{\mathrm{QFT}}_<<<{3} & \gate{\mathrm{P}\,(\mathrm{-\pi})} & \multigate{7}{\mathrm{IQFT\_dg}}_<<<{3} & \gate{\mathrm{X}} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-2} & \qw & \qw\\
	 	\nghost{{a\_c}_{1} :  } & \lstick{{a\_c}_{1} :  } & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \multigate{6}{\mathrm{QFT}}_<<<{3} & \gate{\mathrm{P}\,(\mathrm{0})} & \multigate{6}{\mathrm{IQFT\_dg}}_<<<{3} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_x}_{0} :  } & \lstick{{g\_x}_{0} :  } & \ghost{\mathrm{QFT}} & \gate{\mathrm{X}} & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_x}_{1} :  } & \lstick{{g\_x}_{1} :  } & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_x}_{2} :  } & \lstick{{g\_x}_{2} :  } & \ghost{\mathrm{QFT}} & \gate{\mathrm{X}} & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_y}_{0} :  } & \lstick{{g\_y}_{0} :  } & \ghost{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{8}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{0} & \multigate{2}{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{3\pi}{4}})} & \multigate{2}{\mathrm{IQFT\_dg}}_<<<{0} & \ghost{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{4}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{0} & \multigate{2}{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{3\pi}{2}})} & \multigate{2}{\mathrm{IQFT\_dg}}_<<<{0} & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{1} :  } & \lstick{{g\_y}_{1} :  } & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{4}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\frac{3\pi}{2}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{2}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\pi})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{2} :  } & \lstick{{g\_y}_{2} :  } & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{2}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{\pi})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{-\pi})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{0})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_x} :  } & \lstick{{v\_x} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_y} :  } & \lstick{{v\_y} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_dir\_x} :  } & \lstick{{v\_dir\_x} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-6} & \qw & \qw\\
	 	\nghost{{v\_dir\_y} :  } & \lstick{{v\_dir\_y} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
\\ }}

==> bounceback-near-corner-points.tex <==
\scalebox{0.8}{
\hspace{-5cm}
\Qcircuit @C=1.0em @R=0.2em @!R { \\
	 	\nghost{{a\_v}_{0} :  } & \lstick{{a\_v}_{0} :  } & \qw & \ctrl{1} & \qw \barrier[0em]{14} & \qw & \qw & \ctrl{1} & \qw \barrier[0em]{14} & \qw & \qw & \ctrl{1} & \qw \barrier[0em]{14} & \qw & \qw & \ctrl{1} & \qw \barrier[0em]{14} & \qw & \qw & \ctrl{1} & \qw \barrier[0em]{14} & \qw & \qw & \ctrl{1} & \qw \barrier[0em]{14} & \qw & \qw & \ctrl{1} & \qw \barrier[0em]{14} & \qw & \qw & \ctrl{1} & \qw \barrier[0em]{14} & \qw & \qw & \qw\\
	 	\nghost{{a\_v}_{1} :  } & \lstick{{a\_v}_{1} :  } & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \ctrl{1} & \qw & \qw & \qw & \qw\\
	 	\nghost{{a\_o} :  } & \lstick{{a\_o} :  } & \qw & \targ & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \targ & \qw & \qw & \qw & \qw\\
	 	\nghost{{a\_c}_{0} :  } & \lstick{{a\_c}_{0} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{a\_c}_{1} :  } & \lstick{{a\_c}_{1} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_x}_{0} :  } & \lstick{{g\_x}_{0} :  } & \qw & \ctrl{-4} & \qw & \qw & \qw & \ctrl{-4} & \qw & \qw & \qw & \ctrl{-4} & \qw & \qw & \qw & \ctrl{-4} & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-4} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-4} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-4} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-4} & \gate{\mathrm{X}} & \qw & \qw & \qw\\
	 	\nghost{{g\_x}_{1} :  } & \lstick{{g\_x}_{1} :  } & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_x}_{2} :  } & \lstick{{g\_x}_{2} :  } & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{0} :  } & \lstick{{g\_y}_{0} :  } & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{1} :  } & \lstick{{g\_y}_{1} :  } & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{2} :  } & \lstick{{g\_y}_{2} :  } & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_x} :  } & \lstick{{v\_x} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_y} :  } & \lstick{{v\_y} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_dir\_x} :  } & \lstick{{v\_dir\_x} :  } & \gate{\mathrm{X}} & \ctrl{-3} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-3} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-3} & \qw & \qw & \qw & \ctrl{-3} & \qw & \qw & \qw & \ctrl{-3} & \qw & \qw & \qw & \ctrl{-3} & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-3} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-3} & \gate{\mathrm{X}} & \qw & \qw & \qw\\
	 	\nghost{{v\_dir\_y} :  } & \lstick{{v\_dir\_y} :  } & \qw & \ctrl{-1} & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-1} & \gate{\mathrm{X}} & \qw & \qw & \ctrl{-1} & \qw & \qw & \qw & \qw\\
\\ }}


==> bounceback-reflection-and-streaming.tex <==
\scalebox{.6}{
\hspace{-6cm}
\Qcircuit @C=1.0em @R=0.2em @!R { \\
	 	\nghost{{a\_v}_{0} :  } & \lstick{{a\_v}_{0} :  } & \qw \barrier[0em]{14} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw \barrier[0em]{14} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw \barrier[0em]{14} & \qw & \qw & \qw\\
	 	\nghost{{a\_v}_{1} :  } & \lstick{{a\_v}_{1} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{a\_o} :  } & \lstick{{a\_o} :  } & \ctrl{11} & \qw & \qw & \ctrl{4} & \qw & \qw & \qw & \ctrl{5} & \qw & \qw & \qw & \ctrl{6} & \qw & \qw & \qw & \qw & \ctrl{4} & \qw & \qw & \qw & \ctrl{5} & \qw & \qw & \qw & \ctrl{6} & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{7} & \qw & \qw & \qw & \ctrl{8} & \qw & \qw & \qw & \ctrl{9} & \qw & \qw & \qw & \qw & \ctrl{7} & \qw & \qw & \qw & \ctrl{8} & \qw & \qw & \qw & \ctrl{9} & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{a\_c}_{0} :  } & \lstick{{a\_c}_{0} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{a\_c}_{1} :  } & \lstick{{a\_c}_{1} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_x}_{0} :  } & \lstick{{g\_x}_{0} :  } & \qw & \qw & \multigate{2}{\mathrm{QFT}}_<<<{0} & \control \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \control \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \multigate{2}{\mathrm{IQFT\_dg}}_<<<{0} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_x}_{1} :  } & \lstick{{g\_x}_{1} :  } & \qw & \qw & \ghost{\mathrm{QFT}}_<<<{1} & \qw & \qw & \qw & \qw & \control \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \control \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_x}_{2} :  } & \lstick{{g\_x}_{2} :  } & \qw & \qw & \ghost{\mathrm{QFT}}_<<<{2} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \control \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \control \qw & \qw & \qw & \qw & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{0} :  } & \lstick{{g\_y}_{0} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \multigate{2}{\mathrm{QFT}}_<<<{0} & \control \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \control \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \multigate{2}{\mathrm{IQFT\_dg}}_<<<{0} & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{1} :  } & \lstick{{g\_y}_{1} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ghost{\mathrm{QFT}}_<<<{1} & \qw & \qw & \qw & \qw & \control \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \control \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{2} :  } & \lstick{{g\_y}_{2} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ghost{\mathrm{QFT}}_<<<{2} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \control \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \control \qw & \qw & \qw & \qw & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \qw & \qw & \qw\\
	 	\nghost{{v\_x} :  } & \lstick{{v\_x} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_y} :  } & \lstick{{v\_y} :  } & \qw & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{\frac{\pi}{4}})} \qw & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{\frac{\pi}{2}})} \qw & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{\pi})} \qw & \qw & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{\frac{-\pi}{4}})} \qw & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{\frac{-\pi}{2}})} \qw & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{-\pi})} \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_dir\_x} :  } & \lstick{{v\_dir\_x} :  } & \multigate{1}{\mathrm{2\mbox{-}X}}_<<<{0} & \qw & \qw & \ctrl{-8} & \qw & \qw & \qw & \ctrl{-7} & \qw & \qw & \qw & \ctrl{-6} & \qw & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-8} & \qw & \qw & \qw & \ctrl{-7} & \qw & \qw & \qw & \ctrl{-6} & \qw & \qw & \qw & \gate{\mathrm{X}} & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{\frac{\pi}{4}})} \qw & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{\frac{\pi}{2}})} \qw & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{\pi})} \qw & \qw & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{\frac{-\pi}{4}})} \qw & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{\frac{-\pi}{2}})} \qw & \qw & \qw & \qw & \dstick{\hspace{2.0em}\mathrm{P}\,(\mathrm{-\pi})} \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_dir\_y} :  } & \lstick{{v\_dir\_y} :  } & \ghost{\mathrm{2\mbox{-}X}}_<<<{1} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-6} & \qw & \qw & \qw & \ctrl{-5} & \qw & \qw & \qw & \ctrl{-4} & \qw & \qw & \qw & \gate{\mathrm{X}} & \ctrl{-6} & \qw & \qw & \qw & \ctrl{-5} & \qw & \qw & \qw & \ctrl{-4} & \qw & \qw & \qw & \gate{\mathrm{X}} & \qw & \qw & \qw\\
\\ }}

==> bounceback-wall-reflection.tex <==
\scalebox{.8}{
\hspace{-5cm}
\Qcircuit @C=1.0em @R=0.2em @!R { \\
	 	\nghost{{a\_v}_{0} :  } & \lstick{{a\_v}_{0} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw \barrier[0em]{14} & \qw & \ctrl{2} & \qw & \qw\\
	 	\nghost{{a\_v}_{1} :  } & \lstick{{a\_v}_{1} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{a\_o} :  } & \lstick{{a\_o} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \targ & \qw & \qw\\
	 	\nghost{{a\_c}_{0} :  } & \lstick{{a\_c}_{0} :  } & \multigate{7}{\mathrm{QFT}}_<<<{3} & \gate{\mathrm{P}\,(\mathrm{-\pi})} & \multigate{7}{\mathrm{IQFT\_dg}}_<<<{3} & \gate{\mathrm{X}} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-2} & \qw & \qw\\
	 	\nghost{{a\_c}_{1} :  } & \lstick{{a\_c}_{1} :  } & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \multigate{6}{\mathrm{QFT}}_<<<{3} & \gate{\mathrm{P}\,(\mathrm{0})} & \multigate{6}{\mathrm{IQFT\_dg}}_<<<{3} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_x}_{0} :  } & \lstick{{g\_x}_{0} :  } & \ghost{\mathrm{QFT}} & \gate{\mathrm{X}} & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_x}_{1} :  } & \lstick{{g\_x}_{1} :  } & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_x}_{2} :  } & \lstick{{g\_x}_{2} :  } & \ghost{\mathrm{QFT}} & \gate{\mathrm{X}} & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_y}_{0} :  } & \lstick{{g\_y}_{0} :  } & \ghost{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{8}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{0} & \multigate{2}{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{3\pi}{4}})} & \multigate{2}{\mathrm{IQFT\_dg}}_<<<{0} & \ghost{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{4}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{0} & \multigate{2}{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{3\pi}{2}})} & \multigate{2}{\mathrm{IQFT\_dg}}_<<<{0} & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{1} :  } & \lstick{{g\_y}_{1} :  } & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{4}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\frac{3\pi}{2}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{2}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\pi})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{2} :  } & \lstick{{g\_y}_{2} :  } & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{2}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{\pi})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{-\pi})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{0})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_x} :  } & \lstick{{v\_x} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_y} :  } & \lstick{{v\_y} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_dir\_x} :  } & \lstick{{v\_dir\_x} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-6} & \qw & \qw\\
	 	\nghost{{v\_dir\_y} :  } & \lstick{{v\_dir\_y} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
\\ }}

==> bounceback-wall-reflection2.tex <==

\scalebox{0.8}{
\hspace{-5cm}
\Qcircuit @C=1.0em @R=0.2em @!R { \\
	 	\nghost{{a\_v}_{0} :  } & \lstick{{a\_v}_{0} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw \barrier[0em]{15} & \qw & \ctrl{2} & \qw & \qw\\
	 	\nghost{{a\_v}_{1} :  } & \lstick{{a\_v}_{1} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{a\_o}_{+} :  } & \lstick{{a\_o}_{+} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \targ & \qw & \qw\\
	 	\nghost{{a\_o}_{-} :  } & \lstick{{a\_o}_{-} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{a\_c}_{0} :  } & \lstick{{a\_c}_{0} :  } & \multigate{7}{\mathrm{QFT}}_<<<{3} & \gate{\mathrm{P}\,(\mathrm{-\pi})} & \multigate{7}{\mathrm{IQFT\_dg}}_<<<{3} & \gate{\mathrm{X}} & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-2} & \qw & \qw\\
	 	\nghost{{a\_c}_{1} :  } & \lstick{{a\_c}_{1} :  } & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \multigate{6}{\mathrm{QFT}}_<<<{3} & \gate{\mathrm{P}\,(\mathrm{0})} & \multigate{6}{\mathrm{IQFT\_dg}}_<<<{3} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_x}_{0} :  } & \lstick{{g\_x}_{0} :  } & \ghost{\mathrm{QFT}} & \gate{\mathrm{X}} & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_x}_{1} :  } & \lstick{{g\_x}_{1} :  } & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_x}_{2} :  } & \lstick{{g\_x}_{2} :  } & \ghost{\mathrm{QFT}} & \gate{\mathrm{X}} & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \ghost{\mathrm{QFT}} & \qw & \ghost{\mathrm{IQFT\_dg}} & \qw & \qw & \qw & \qw & \ctrl{-1} & \qw & \qw\\
	 	\nghost{{g\_y}_{0} :  } & \lstick{{g\_y}_{0} :  } & \ghost{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{8}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{0} & \multigate{2}{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{3\pi}{4}})} & \multigate{2}{\mathrm{IQFT\_dg}}_<<<{0} & \ghost{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{4}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{0} & \multigate{2}{\mathrm{QFT}}_<<<{0} & \gate{\mathrm{P}\,(\mathrm{\frac{3\pi}{2}})} & \multigate{2}{\mathrm{IQFT\_dg}}_<<<{0} & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{1} :  } & \lstick{{g\_y}_{1} :  } & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{4}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\frac{3\pi}{2}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{2}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \ghost{\mathrm{QFT}}_<<<{1} & \gate{\mathrm{P}\,(\mathrm{\pi})} & \ghost{\mathrm{IQFT\_dg}}_<<<{1} & \qw & \qw & \qw & \qw\\
	 	\nghost{{g\_y}_{2} :  } & \lstick{{g\_y}_{2} :  } & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{\frac{-3\pi}{2}})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{\pi})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{-\pi})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \ghost{\mathrm{QFT}}_<<<{2} & \gate{\mathrm{P}\,(\mathrm{0})} & \ghost{\mathrm{IQFT\_dg}}_<<<{2} & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_x} :  } & \lstick{{v\_x} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_y} :  } & \lstick{{v\_y} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
	 	\nghost{{v\_dir\_x} :  } & \lstick{{v\_dir\_x} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \ctrl{-6} & \qw & \qw\\
	 	\nghost{{v\_dir\_y} :  } & \lstick{{v\_dir\_y} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
\\ }}

